The paradox of the compositionality of natural language: a neural machine translation case study

Obtaining human-like performance in NLP is often argued to require compositional generalisation. Whether neural networks exhibit this ability is usually studied by training models on highly compositional synthetic data. However, compositionality in natural language is much more complex than the rigid, arithmetic-like version such data adheres to, and artificial compositionality tests thus do not allow us to determine how neural models deal with more realistic forms of compositionality. In this work, we re-instantiate three compositionality tests from the literature and reformulate them for neural machine translation (NMT). Our results highlight that: i) unfavourably, models trained on more data are more compositional; ii) models are sometimes less compositional than expected, but sometimes more, exemplifying that different levels of compositionality are required, and models are not always able to modulate between them correctly; iii) some of the non-compositional behaviours are mistakes, whereas others reflect the natural variation in data. Apart from an empirical study, our work is a call to action: we should rethink the evaluation of compositionality in neural networks and develop benchmarks using real data to evaluate compositionality on natural language, where composing meaning is not as straightforward as doing the math.

==> tables/global_compositionality_table.tex <==
\begin{table}[!ht]
\centering\small\setlength{\tabcolsep}{4pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{clccccc}
\toprule
\textbf{Freq.} & \textbf{Idiom} & \textbf{Synth.} & \textbf{Semi-Nat.} & \textbf{Nat.} \\ \midrule\midrule
1173 & out of the \underline{blue} & .00\pms{.00} & .00\pms{.00} & .02 \\
456 & call it a \underline{night} & .44\pms{.20} & .95\pms{.12} & .03 \\
384 & back to \underline{square} one & .00\pms{.00} & .02\pms{.06} & .01 \\
383 & \underline{icing} on the cake & .56\pms{.06} & .20\pms{.11} & .35 \\
190 & kill two \underline{birds} (\dots) & .82\pms{.11} & .91\pms{.13} & .09 \\
190 & spill the \underline{beans} & 1.00\pms{.00} & 1.00\pms{.01} & .91 \\
187 & \underline{nest egg} & .95\pms{.06} & 1.00\pms{.00} & .79 \\
154 & turn a \underline{deaf ear} & 1.00\pms{.00} & .87\pms{.08} & .35 \\
125 & the drop of a \underline{hat} & 1.00\pms{.00} & 1.00\pms{.00} & .93 \\
115 & kick the \underline{bucket} & 1.00\pms{.00} & 1.00\pms{.01} & .98 \\
97 & shake a \underline{leg} & 1.00\pms{.00} & 1.00\pms{.00} & .87 \\
79 & the whole \underline{nine yards} & 1.00\pms{.00} & .84\pms{.10} & .46 \\
72 & hit the \underline{hay} & 1.00\pms{.00} & 1.00\pms{.01} & .92 \\
71 & add \underline{insult} to \underline{injury} & .81\pms{.14} & .70\pms{.07} & .32 \\
70 & raining \underline{cats} and \underline{dogs} & 1.00\pms{.00} & 1.00\pms{.01} & 1.00 \\
37 & life in the fast \underline{lane} & 1.00\pms{.00} & 1.00\pms{.00} & .94 \\
35 & bird in the hand is  & 1.00\pms{.00} & 1.00\pms{.01} & .82 \\
& worth \underline{two} in the \underline{bush} \\
24 & \underline{birds} of a \underline{feather} (\dots) & 1.00\pms{.00} & 1.00\pms{.01} & 1.00 \\
24 & once \underline{bitten}, twice \underline{shy} & 1.00\pms{.00} & 1.00\pms{.01} & .92 \\
15 & haste makes \underline{waste} & 1.00\pms{.00} & 1.00\pms{.00} & .93 \\
\bottomrule
\end{tabular}}
\caption{Performance in the global compositionality test, measured using the overgeneralisation metric that expresses the number of samples with a local translation of the idiom. Idiom keywords are underlined.}
\label{tab:overgeneralisation_results}
\end{table}

==> tables/substitutivity_all.tex <==
\begin{tabular}{lcccc}
 & Synthetic & Semi-natural & Natural & \% of total \\
One synonym untranslated & 7 & 9 & 18 & 10\\
One synonym wrongly translated & 6 & 3 & 6 & 4\\
Both synonyms wrongly translated & 3 & 2 & 7 & 3\\
Different synonym translation & 3 & 3 & 5 & 3\\\hline
Target errors & 20 & 23 & 30 & 21\\
Rephrasing & 46 & 56 & 44 & 42\\
Source ambiguities & 10 & 5 & 2 & 5\\
Changes in punctuation & 19 & 18 & 5 & 12\\
\end{tabular}

==> tables/substitutivity_results.tex <==
\begin{table}[!t]
\small\setlength{\tabcolsep}{4pt}
\centering
% \begin{subtable}[b]{\columnwidth}\centering
\resizebox{\columnwidth}{!}{\begin{tabular}{llcccccc}
\toprule
\textbf{Synonym} & %& \multicolumn{3}{l}{\textbf{Consistency}} \\ 
& \textbf{Synthetic} & \textbf{Semi-Nat.} & \textbf{Natural} \\ \midrule \midrule
\textit{- Spelling} \\
aeroplane & airplane & .95\pms{.02} & .63\pms{.09} & .60  \\
aluminium & aluminum & .92\pms{.03} & .66\pms{.06} & .53  \\
doughnut & donut & .98\pms{.02} & .80\pms{.05} & .86  \\
foetus & fetus & .81\pms{.10} & .65\pms{.05} & .62  \\
flautist & flutist &  .09\pms{.10} & .04\pms{.05} & .26  \\
lasagne & lasagna & .46\pms{.30} & .69\pms{.09} & .73  \\
moustache & mustache & .92\pms{.08} & .67\pms{.11} & .85  \\
tumour & tumor & .87\pms{.07} & .54\pms{.10} & .53  \\
pyjamas & pajamas & .74\pms{.15} & .48\pms{.09} & .64  \\
sulphur & sulfur & .96\pms{.02} & .66\pms{.10} & .57  \\
yoghurt & yogurt & .58\pms{.20} & .53\pms{.15} & .69  \\
\vspace{-2.7mm}\\
\hdashline
\vspace{-2.7mm}\\
\multicolumn{2}{c}{\textit{Mean}} & .75\pms{.26} & .58\pms{.19} & .63\pms{.16} \\
\multicolumn{2}{c}{\textit{Mean synonym only}} & .92\pms{.26} & .91\pms{.27} & .94\pms{.16} \\%\midrule
\bottomrule
\textit{- Term} \\
aubergine & eggplant & .76\pms{.16} & .67\pms{.06} & .69  \\
milliard & billion & .00\pms{.00} & .00\pms{.00} & .16  \\
candyfloss & cotton can. & .00\pms{.00} & .00\pms{.00} & .01  \\
courgette & zucchini & .90\pms{.13} & .27\pms{.12} & .69  \\
football & soccer & .63\pms{.20} & .60\pms{.21} & .41  \\
holiday & vacation & .84\pms{.07} & .62\pms{.04} & .62  \\
ladybird & ladybug & .80\pms{.06} & .69\pms{.07} & .83  \\
postcode & zip code & .94\pms{.02} & .75\pms{.05} & .69  \\
catapult & slingshot & .94\pms{.05} & .61\pms{.11} & .65  \\
\vspace{-2.7mm}\\
\hdashline
\vspace{-2.7mm}\\
\multicolumn{2}{c}{\textit{Mean}} & .64\pms{.36} & .47\pms{.28} & .53\pms{.26} \\
\multicolumn{2}{c}{\textit{Mean synonym only}} & .74\pms{.41} & .76\pms{.41} & .74\pms{.32} \\
\bottomrule
\end{tabular}}
    \caption{Substitutivity results for full translation and synonym only, measured with the consistency metric. %for the full translation and the synonym only.
    }\label{tab:substitutivity_results}
\end{table}




==> tables/substitutivity_small.tex <==
\begin{tabular}{lcccc}
 & Synthetic & Semi-natural & Natural & \% of total \\
One synonym untranslated & 9 & 5 & 18 & 9\\
One synonym wrongly translated & 9 & 7 & 4 & 6\\
Both synonyms wrongly translated & 9 & 8 & 12 & 8\\
Different synonym translation & 5 & 1 & 8 & 4\\\hline
Target errors & 10 & 11 & 29 & 14\\
Rephrasing & 42 & 71 & 46 & 45\\
Source ambiguities & 9 & 1 & 0 & 3\\
Changes in punctuation & 17 & 19 & 2 & 11\\
\end{tabular}

==> tables/substitutivity_tiny.tex <==
\begin{tabular}{lcccc}
 & Synthetic & Semi-natural & Natural & \% of total \\
One synonym untranslated & 11 & 13 & 28 & 12\\
One synonym wrongly translated & 13 & 6 & 11 & 7\\
Both synonyms wrongly translated & 6 & 10 & 12 & 7\\
Different synonym translation & 0 & 0 & 0 & 0\\\hline
Target errors & 69 & 60 & 66 & 47\\
Rephrasing & 23 & 39 & 29 & 22\\
Source ambiguities & 8 & 1 & 0 & 2\\
Changes in punctuation & 4 & 5 & 3 & 3\\
\end{tabular}

==> tables/synonyms.tex <==
\begin{table}[!t]
\small\centering
\begin{tabular}{ll|ll}
    \toprule
    \multicolumn{2}{l|}{\textbf{Spelling Differences}} & \multicolumn{2}{l}{\textbf{Term Differences}} \\
    \textit{British} & \textit{American} & \textit{British} & \textit{American} \\ \midrule \midrule
    aeroplane & airplane & aubergine & eggplant  \\
    aluminium & aluminum & milliard & billion  \\
    doughnut & donut & candyfloss & cotton candy \\
    foetus & fetus & courgette & zucchini \\
    flautist & flutist & football & soccer   \\
    moustache & mustache  & holiday & vacation   \\
    tumour & tumor  & ladybird & ladybug \\
    pyjamas & pajamas  & postcode & zip code  \\
    sulphur & sulfur   & catapult & slingshot  \\
    yoghurt & yogurt \\
    lasagna & lasagne \\
    \bottomrule
\end{tabular}
    \caption{Synonyms used for the substitutivity compositionality test, with 11 pairs of synonymous words with a different spelling in British and American English and 9 pairs of synonymous words with a major term change between British and American English.}\label{tab:synonyms}
\end{table}


==> tables/systematicity_all.tex <==
\begin{tabular}{lccccccc}
& \multicolumn{2}{c}{Synthetic} & \multicolumn{2}{c}{semi-natural} & \multicolumn{2}{c}{natural} & Avg \% of all \\
& S1p & S3 & S1p & S3 & S1p & S3 & \\\hline
Target errors & 22 & 26 & 34 & 34 & 26 & 40 & 27\\
Rephrasing & 36 & 78 & 70 & 44 & 64 & 68 & 54\\
Source ambiguities & 38 & 8 & 0 & 18 & 4 & 4 & 11\\
Changes in punctuation & 8 & 8 & 4 & 14 & 6 & 10 & 8\\
\end{tabular}


% {"Target errors": [22, 26, 34, 34, 26, 40, 27],
% "Rephrasing": [36, 78, 70, 44, 64, 68, 54],
% "Source ambiguities": [38, 8, 0, 18, 4, 4,,11],
% "Changes in punctuation": [8, 8, 4, 14, 6, 10, 8]}
% 
% 
% {"Target errors": [36, 44, 50, 40, 32, 47, 37], 
% "Rephrasing": [40, 56, 54, 30, 66, 69, 46], 
% "Source ambiguities": [30, 8, 4, 28, 6, 10, 13], 
% "Changes in punctuation": [12, 0, 4, 12, 0, 4, 5]}


==> tables/systematicity_small.tex <==
\begin{tabular}{lccccccc}
 & \multicolumn{2}{c}{Synthetic} & \multicolumn{2}{c}{semi-natural} & \multicolumn{2}{c}{natural} & Avg \% of all \\
& S1p & S3 & S1p & S3 & S1p & S3 & \\\hline
Target errors & 36 & 44 & 50 & 40 & 32 & 47 & 37\\
Rephrasing & 40 & 56 & 54 & 30 & 66 & 69 & 46\\
Source ambiguities & 30 & 8 & 4 & 28 & 6 & 10 & 13\\
Changes in punctuation & 12 & 0 & 4 & 12 & 0 & 4 & 5\\
\end{tabular}

==> tables/systematicity_tiny.tex <==
\begin{tabular}{lccccccc}
 & \multicolumn{2}{c}{Synthetic} & \multicolumn{2}{c}{semi-natural} & \multicolumn{2}{c}{natural} & Avg \% of all \\
& S1p & S3 & S1p & S3 & S1p & S3 & \\\hline
Target errors & 71 & 74 & 83 & 72 & 78 & 124 & 62\\
Rephrasing & 22 & 28 & 41 & 18 & 38 & 32 & 22\\
Source ambiguities & 24 & 10 & 9 & 38 & 18 & 8 & 13\\
Changes in punctuation & 4 & 4 & 5 & 1 & 4 & 2 & 2\\
\end{tabular}
